Run Time Assurance for Simultaneous Constraint Satisfaction During Spacecraft Attitude Maneuvering

A fundamental capability for On-orbit Servicing, Assembly, and Manufacturing (OSAM) is inspection of the vehicle to be serviced, or the structure being assembled. This research assumes autonomous slewing to maintain situational awareness of multiple vehicles operating in close proximity where several safety constraints must be satisfied. A variety of techniques may be used as the primary controller. The focus of this research is developing Run Time Assurance (RTA) filters that monitor system behavior and the output of the primary controller to enforce safety constraint satisfaction. Specifically, this research explores combining a subset of the constraints into an Active Set Invariance Filter (ASIF) RTA defined using control barrier functions. This method is minimally invasive to the primary control by minimizing deviation from the desired control output of the primary controller, while simultaneously enforcing all safety constraints. The RTA is designed to ensure the spacecraft maintains attitude requirements for communication and data transfer with a ground station during scheduled communication windows, adheres to conical attitude keep out zones, limits thermally unfavorable attitude duration, maintains attitude requirements for sufficient power generation, ensures maneuvers are below threshold to cause structural damage, ensures maximum angular velocity is below limits to maintain ability to respond quickly to new slewing commands, and conserves actuator use to prevent wear when possible. Slack variables are introduced into the ASIF controller to prioritize safety constraints when a solution to all safety constraints is infeasible. Monte Carlo simulation results as well as plots of example cases are shown and evaluated for a three degree of freedom spacecraft with reaction wheel attitude control.

==> Main_obs_6dof.tex <==
% % IEEEAerospace2012.cls requires the following packages: times, rawfonts, oldfont, geometry
% \documentclass[twocolumn,letterpaper]{IEEEAerospaceCLS}  % only supports two-column, letterpaper format

% % The next line gives some packages you may find useful for your paper--these are not required though.
% %\usepackage[]{graphicx,float,latexsym,amssymb,amsfonts,amsmath,amstext,times,psfig}
% % NOTE: The .cls file is now compatible with amsmath!!!

% \usepackage[]{graphicx}    % We use this package in this document
% \usepackage{amsfonts}
% \newcommand{\ignore}[1]{}  % {} empty inside = %% comment

% \usepackage{xurl} % allows break in url so it doesnt run into next column
% \usepackage{amsmath}
% \DeclareMathOperator*{\argmin}{argmin} % thin space, limits underneath in displays
% \DeclareMathOperator*{\infin}{inf} % thin space, limits underneath in displays
% \usepackage{amsmath,amsfonts,amsthm,bm} % Math packages


% \begin{document}
% \title{Run Time Assured Reinforcement Learning for Spacecraft Maneuvering}

% \author{
% Cassie-Kay McQuinn\\ 
% Department of Aerospace Engineering\\
% Texas A\&M University\\
% College Station, TX, 77843\\
% ckmcquinn@tamu.edu
% \and 
% Kyle Dunlap\\
% Parallax Advanced Research\\
% 4035 Colonel Glenn Hwy\\
% Beavercreek, OH, 45431 \\
% kyle.dunlap@parallaxresearch.org
% \and 
% Nathaniel Hamilton\\
% Parallax Advanced Research\\
% 4035 Colonel Glenn Hwy\\
% Beavercreek, OH, 45431 \\
% nathaniel.hamilton@parallaxresearch.org
% \and
% Jabari Wilson\\
% Department of Mechanical Engineering\\
% University of Florida\\
% Gainesville, Florida, 32611\\
% jabari.wilson@outlook.com
% \and
% Kerianne L. Hobbs\\ 
% Air Force Research Laboratory\\
% 2241 Avionics Circle\\
% Wright-Patterson AFB, OH, 45433\\
% kerianne.hobbs@us.af.mil
% %%%% IMPORTANT: Use the correct copyright information--IEEE, Crown, or U.S. government. %%%%%
% \thanks{\footnotesize 979-8-3503-0462-6/24/$\$31.00$ \copyright2024 IEEE}              % This creates the copyright info that is the correct 2024 data.
% %\thanks{{U.S. Government work not protected by U.S. copyright}}         % Use this copyright notice only if you are employed by the U.S. Government.
% %\thanks{{979-8-3503-0462-6/24/$\$31.00$ \copyright2024 Crown}}          % Use this copyright notice only if you are employed by a crown government (e.g., Canada, UK, Australia).
% %\thanks{{979-8-3503-0462-6/24/$\$31.00$ \copyright2024 European Union}}    % Use this copyright notice is you are employed by the European Union.
% }



% \maketitle

% \thispagestyle{plain}
% \pagestyle{plain}



% \maketitle

% \thispagestyle{plain}
% \pagestyle{plain}

% \begin{abstract}

% A fundamental capability for On-orbit Servicing, Assembly, and Manufacturing (OSAM) is inspection of the vehicle to be serviced, or the structure being assembled. This research investigates autonomous slewing to maintain situational awareness of multiple vehicles operating in close proximity where several safety constraints must be satisfied. A reinforcement learning solution is used as a primary controller to command slewing. Run time assurance (RTA) monitors system behavior and the output of the neural network control system trained using reinforcement learning to enforce safety constraint satisfaction during training as well as during testing. This research explores combining a subset of the constraints into an Active Set Invariance Filter (ASIF) RTA defined using control barrier functions that is minimally invasive to the primary control, by minimizing deviation from the desired control output of the neural network control system, while simultaneously enforcing all safety constraints. The RTA is designed to ensure the spacecraft maintains attitude requirements for communication and data transfer with a ground station during scheduled communication windows, adheres to conical attitude keep out zones, limits thermally unfavorable attitude duration, maintains attitude requirements for sufficient power generation, ensures maneuvers are below threshold to cause structural damage, ensures maximum angular velocity is below limits to maintain ability to respond quickly to new slewing commands, and conserves actuator use to prevent wear when possible. Simulation results are shown and evaluated for a six degree of freedom spacecraft with thrusters and reaction wheel attitude control. 

% \end{abstract} 


% \tableofcontents

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Introduction}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % discuss background of safe RL, RTA. Why its important and what has currently been done. Previous work has satisfied one control barrier function but this work aims to satisfy multiple as well as priority rank?
% % background on mission - Vehicle inspection 
% % On-orbit Servicing Assembly and Manufacturing (OSAM) 
% % why do we care about RL

% % OSAM source? can include example of OSAM such as ISS, Hubble telescope, and Mission Extension Vehicles

% % this is only those registered with UNOOS, need a way to say that there are likely more
% According to the United Nation's Register of Objects Launched into Outer Space \cite{OSOidx}, 2474 registered objects were launched into outer space in 2022. Comparing this to the 222 registered objects that were launched in 2015, the space industry is growing at a rapid pace. With this growth comes a change in the manner with which missions are conducted, introducing a paradigm shift with the emerging technology of On-orbit Servicing, Assembly, and Manufacturing (OSAM) \cite{arney2021orbit}. OSAM will facilitate extended space missions, orbital manipulation of existing objects, such as the removal of space debris, and repair of existing satellite systems. A major capability of OSAM is the inspection task. Inspection is the observation of systems to analyze features of interest, including damaged assets or assembly of new  components. Inspection vehicles must maintain situational awareness of multiple vehicles operating in close proximity. Additionally, safety and mission constraints on the inspection vehicle must be satisfied for the vehicle to successfully complete the inspection task. \\
% A safe set of states are formed where all the constraints. Due to the multiple constraints deriving a controller that keeps the spacecraft within the set for all time using traditional control techniques. Through trail-and-error search, Reinforcement Learning (RL) determines, or \textit{learns}, which actions maximize a reward \cite{sutton2018reinforcement}. For autonomous spacecraft operations, this enables high performance for low online computational complexity. In RL, training occurs offline during the design phase, then a 


% Building off of the work \cite{dunlap2023run} and \cite{dunlap2023run2}, this research will utilize Run Time Assurance (RTA) during RL training in order to enforce assurance to multiple safety constraints. 

% investigate training with ASIF RTA due to the complexity of the constraints, it would be very difficult to determine a backup control law that satisfies all constraints.

% % other approches to solving this problem 
% % SOMETHING ABOUT DERVING A CONTROLLER BEING DIFFICULT BECAUSE OF ALL THE REQUIREMENTSadmin/manage/my-submissions
% % something about need for autonomy, can incorporate RL controller here

% The concept of safety....

% %"The concept of safety is fundamentally linked to the idea of constrained behavior" -ASIF paper


% % something about requirements of a system being satisfied, can incorporate need for RTA here

% % sentance about this work will 



% % why do we care about RTA
% % discuss the 4 main types of RTA systems here or in RTA section?
% % specify that its explicit RTA, why explicit rather than implicit?
% The contribution of this paper is the application of ASIF RTA, in training and testing, to enforce multiple safety constraints to a spacecraft with attitude and translational control. The neural network is trained with ASIF RTA active to prevent the system from entering unsafe states. Then the controller is simulated on the spacecraft with ASIF RTA active to ensure adheres to the safety constraints. 

% % key points:
% % safety - RTA
% % RL controller
% % 
% This paper is organized as follows: 
% % Section 2: RTA
% % somewhere need to incorporate slack variables/constraint prioritization
% % Section 3: RL
% % Section 3: Spacecraft attitude representation/Methodology
% % Section 4: Simulation Results
% % Section 5: Conclusions
 


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Run Time Assurance}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This work considers a continuous-time control affine system defined as
% \begin{equation}\label{e:dynamics}
%     {\bm{\dot{x}}}=  f({\bm{x}})+ g({\bm{x}}){\bm{u}}
% \end{equation}
% where $\bm{x} \in \mathcal{X} \subseteq $ ${\mathbb{R}} ^ {n}$  denotes the state vector, ${\bm{u}} \in {\mathcal{U}} \subseteq {\mathbb{R}}^{m}$ denotes the control vector, and $f : \mathcal{X} \rightarrow  $ ${\mathbb{R}} ^ {n}$  and $g : \mathcal{X} \rightarrow $ ${\mathbb{R}} ^ {n \times m}$  are locally Lipschitz continuous functions. Here, $\mathcal{X}$ is the set of all possible state values and $\mathcal{U}$ is the admissible control set.\\
% RTA is an online safety assurance technique that filters the control inputs from a primary controller to preserve safety of the system. RTA filters are decoupled from the primary controller. This enabled the objective of the primary controller be to achieve the highest performance while the objective of the RTA filter is to assure safety. The RTA filter intercepts the desired control $\bm{u}_{des}$ from the primary controller, modifies it as necessary to assure safety, and then passes a new action $\bm{u}_{act}$ to the plant. A feedback control system with RTA is shown in figure \ref{rta_cl}.\\
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=3.25in]{Figures/RTAcontrolLoop.png}
%     \caption{Control Loop with RTA}
%     \label{rta_cl}
% \end{figure}
% The Active Set Invariance Filter (ASIF) RTA \cite{gurriet2018online} is an optimization-based technique designed to be minimally invasive towards the primary controller. ASIF algorithms use Control Barrier Functions (CBF) \cite{ames2019control} to enforce adherence to safety constraints. The ASIF algorithm used in this work is defined as
% \begin{equation}\label{e:ASIF}
%     \begin{gathered}
%     {\bm{u}}_{act}({\bm{x}},{\bm{u}}_{des}) = \argmin_{{\bm{u}} \in \mathcal{U}} \lvert \lvert {\bm{u}}_{des} - {\bm{u}} \rvert \rvert ^2 \\
%      \text{s.t. } BC_i({\bm{x}}, {\bm{u}}) \geq 0, \forall i\in \{1,..., M \} 
%     \end{gathered}
% \end{equation}
% ASIF uses a Quadratic Program (QP) to minimize the $l^2$ norm difference between ${\bm{u}}_{des}$ and ${\bm{u}}_{act}$, and therefore only modifies ${\bm{u}}_{des}$ when necessary to assure safety. The inequality constraint for the QP are a set of $M$ Barrier Constraints (BC). To define safety of the system, consider a set of $M$ continuously differentiable functions $h_i : {\mathcal{X}} \rightarrow {\mathbb{R}}, \forall i \in \{1,...,M\}$, then the safe set, $\mathcal{C}_S$, can be defined as,
% \begin{equation}
%     {\mathcal{C}}_S := \{ {\bm{x}} \in {\mathcal{X}} \lvert h_i({\bm{x}}) \geq 0, \forall i \in \{1,...,M \}.
% \end{equation}
% Note, this work focuses on safety defined explicitly rather than implicitly. Explicit safe sets are defined offline. Implicit safe sets are determined by evaluating trajectories using a predefined backup control law to evaluate if a given input will result in the system leaving the safe set. The system is considered safe if $\mathcal{C}_S$ is forward invariant with respect to Eq. \ref{e:dynamics}, such that, 
% \begin{equation}
%     {\bm{x}} ({t}_0) \in  {\mathcal{C}}_S \Rightarrow {\bm{x} }(t) \in{} {\mathcal{C}}_S , \forall{} \geq{} t_0.
% \end{equation}
% Barrier constraints, which are satisfied when $BC_i({\bm{x}},{\bm{u}}) \geq 0$, enforce Nagumo's condition \cite{nagumo1942lage}.
% The boundary of the set is formed by $h_i(\bm{x})$ and, if $\dot{h}_i(\bm{x})$ is never decreasing, then $\bm{x}$ will never leave the safe set ${\mathcal{C}}_S$. Since the boundary of a set does not have volume, a strengthening class-$\kappa$ infinity function, $\alpha$, is utilized to enforce the boundary condition. The resulting BC is defined as,
% \begin{equation}
%     BC({\bm{x}},{\bm{u}}) = \dot{h}({\bm{x}},{\bm{u}})+\alpha (h({\bm{x}}))
% \end{equation}
% where $\dot{h}({\bm{x}})$ is defined as,
% \begin{equation}
%     \dot{h}({\bm{x}})=\nabla h({\bm{x}})\dot{{\bm{x}}} = L_f h({\bm{x}})+L_g h({\bm{x}}) {\bm{u}} \geq 0,
% \end{equation}
% where $L_f$ and $L_g$ are Lie derivatives of $h_i$ along $f$ and $g$ respectively. Using Eq. \ref{e:dynamics}, the BC becomes,
% \begin{equation}\label{e:BC}
%     BC({\bm{x}},{\bm{u}}):=\nabla h({\bm{x}})(f({\bm{x}})+ g({\bm{x}}){\bm{u}}) + \alpha (h({\bm{x}}))
% \end{equation}
% \subsection{High Order Control Barrier Functions}
% For some constraints, $\nabla h({\bm{x}})$ may not depend on the control input. In this case, the BC is not valid as $\nabla h({\bm{x}})g({\bm{x}}){\bm{u}}=0$. To solve this problem, High Order Control Barrier Functions (HOCBF) can be used to differentiate the constraint and allow $\nabla h({\bm{x}})$ to depend on $\bm{u}$. A sequence of functions ${{\Psi}}_j: {\mathbb{R}}^n \rightarrow {\mathbb{R}}, \forall j \in \{1,...,m\}$ is defined as,
% \begin{equation}\label{e:HOBC}
%     {{\Psi}}_j({\bm{x}}):=\dot{{{\Psi}}}_{j-1}({\bm{x}}) + \alpha_j({{\Psi}}_j({\bm{x}})), \forall j \in \{1,...,m\},
% \end{equation}
% where $m$ us referred to as the relative degree of the system and is the number of times needed to differentiate the constraint in order for the control to explicitly appear in the corresponding derivative \cite{xiao2022control}. In this case, $\Psi_0({\bm{x}}) = h({\bm{x}})$ and $\dot{\Psi}({\bm{x}})g({\bm{x}}) \neq 0$. In the cases where $j<m, \dot{\Psi}({\bm{x}}))=\nabla\Psi({\bm{x}})f({\bm{x}})$. Also note that when $m=1, \Psi({\bm{x}})$ is equivalent to Eq. \ref{e:BC}.
% \subsection{Slack Variables}
% When simulating a system with multiple safety constraints, there can be situations or conditions in which these constraints conflict with each other. This will cause the QP to fail if it can not find a solution without violating a constraint. In order to prevent this from occurring, a slack variable $\delta$ can be added into Eq. \ref{e:ASIF} such that it becomes 
% \begin{equation}\label{e:ASIF_slack}
%     \begin{gathered}
%     {\bm{u}}_{act}({\bm{x}},{\bm{u}}_{des}) = \argmin_{{\bm{u}},\delta \in \mathcal{U}} \lvert \lvert {\bm{u}}_{des} - {\bm{u}} \rvert \rvert ^2 + \sum_ip_i\delta_i^2 \\
%      \text{s.t. } BC_i({\bm{x}}, {\bm{u}}) \geq \delta_i, \forall i\in \{1,..., M \} 
%     \end{gathered}
% \end{equation}
% The QP also solves for the slack variables which adds a buffer on the constraint. $p$ is a hyper-parameter that correlates to a scaling constant on the slack variable. Its value should be large (for example $10^{12}$) such that the slack variable is only non zero in the case that the QP cannot be solved. For the QP to have a unique solution, there can be $M-1$ slack variables, meaning at least one constraint cannot have a slack variable. Including slack variables relaxes the constraint, so it should only be included on constraints that can be violated or the lowest priority constraints.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Reinforcement Learning Control Law}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Problem Formulation}\label{s:pf}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The inspection problem consists of an active "deputy" spacecraft that is inspecting a passive "chief" in a linearized relative-motion reference frame. This sections describes the dynamics of the system and the constraints that are used to enforce safety. The neural network controller learns how to inspect the chief spacecraft through RL while the ASIF RTA ensures safety constraints are not violated. 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=2.5in]{Figures/cubeSat.png}
%     \caption{Hypothetical Cubesat.}
%     \label{f:cube_sat}
% \end{figure}
% \subsection{Dynamics}
% The deputy spacecraft is modeled as a 6U CubeSat as shown in Figure \ref{f:cube_sat} with the body reference frame ${\mathcal{F}}_B:=({\mathcal{O}}_B,\hat{i}_B,\hat{j}_B,\hat{k}_B)$. The spacecraft has an antenna on the $+\hat{j}_B$ face for communication with a ground station, a sensor for inspecting the chief on the $+\hat{i}_B$ face, and a solar panel on the $+\hat{k}_B$ face. The system dynamics are represented in Hill's reference frame \cite{hill1878researches}, ${\mathcal{F}}_H:=({\mathcal{O}}_H,\hat{i}_H,\hat{j}_H,\hat{k}_H)$, with the origin $O_H$ centered on the chief spacecraft in a circular orbit around Earth. As shown in Figure \ref{f:hill_frame}, the unit vector $\hat{i}_H$ points from the center of the chief spacecraft away from the center of the Earth, $\hat{j}_H$ points in the direction of motion of the chief spacecraft around the Earth, and $\hat{k}_H$ is normal to $\hat{i}_H$ and $\hat{j}_H$. For this problem, the chief spacecraft is assumed to remain in the same circular orbit in Low Earth Orbit (LEO). The deputy spacecraft maneuvers relative to the chief spacecraft with orientation control via a three wheel reaction wheel array, where the reaction wheels are aligned with the principal, and translation control via three thrusters that are each aligned to a principal axis. 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=1\linewidth]{Figures/HillsFrame_CD2.png}
%     \caption{Hill's Reference Frame.}
%     \label{f:hill_frame}
% \end{figure}
% This subsection outlines the dynamical models used for the attitude, translational, surface temperature, and stored energy of the spacecraft as well as the dynamics for the sun in the simulation.
% \subsubsection{Attitude}
% The attitude of the deputy spacecraft is modeled in the principal axis body reference frame, where the origin, ${\mathcal{O}}_B$ is located at the center of mass of the spacecraft, and the axes are aligned with the eigenvectors of the spacecraft inertia matrix. The attitude is then modeled using a quaternion formulation \cite{markley2014fundamentals}, which represents a rotation between two reference frames. In this case, the quaternion is used to represent the rotation of the spacecraft from Hill's reference frame to the body reference frame. The quaternion also avoids singularity points that arise from Euler angles. A quaternion ${\mathbf{q}} \in {\mathbb{R}}^4$ is comprised of a three vector part ${\mathbf{q}}_v= {\mathbf{q}}_{1:3}$ and a scalar part $q_4$. The angular rates ${\bm{\omega}} \in {\mathbb{R}}^3$ are then used to represent the rotation of the spacecraft about each of its principal axes. The derivative of the angular rates is given by Euler's rotation equations,
% \begin{equation}\label{e:eulerRot}
%     {\mathbf{J}\dot{\bm{\omega}}+\bm{\omega} \times \bf{J}\bm{\omega} = \bm{\tau}},
% \end{equation}
% where $\mathbf{J}$ is the spacecraft's inertia matrix and $\bm{\tau}$ is the torque applied to the spacecraft via the reaction wheels. Therefore, ${\bm{\tau}} = D{\dot{\bm{\psi}}}$, where $D$ is the reaction wheel spin axis mass moment of inertia and ${\dot{\bm{\psi}}}$ is the reaction wheel acceleration. Eq. \ref{e:eulerRot} can then be written in the principal axis body reference frame as,
% \begin{equation}
%     \begin{bmatrix} 
%         \dot{\omega}_1 \\ \dot{\omega}_2 \\ \dot{\omega}_3
%     \end{bmatrix} =
%     \begin{bmatrix}
%         J_1^{-1}((J_2-J_3)\omega_1\omega_3+D\dot{\psi}_1) \\ J_2^{-1}((J_3-J_1)\omega_2\omega_3+D\dot{\psi}_2) \\ J_3^{-1}((J_1-J_2)\omega_1\omega_2+D\dot{\psi}_3)
%     \end{bmatrix}
% \end{equation}
% Here, $J_1,J_2,$ and $J_3$ are the principal moments of inertia of the spacecraft. The relation of the quaternion derivatives to the angular rates is given by,
% \begin{equation}
%     {\mathbf{\dot{q}}} = \frac{1}{2}{\mathbf{\Xi}}(\mathbf{q})\bm{\omega}
% \end{equation}
% where $\mathbf{\Xi}$ is given by,
% \begin{equation}
%     {\mathbf{\Xi}}({\mathbf{q}})=\begin{bmatrix}
%         q_s{\mathcal{I}}-{\mathbf{q}}_v^\chi \\ -{\mathbf{q}}_v^T
%     \end{bmatrix} = \begin{bmatrix}
%         q_4 & -q_3 & q_2 \\ q_3 & q_4 & -q_1 \\ -q_2 & q_1 & q_4 \\ -q_1 & -q_2 & -q_3
%     \end{bmatrix}
% \end{equation}
% where ${\mathcal{I}} \in {\mathbb{R}}^3$ represents the identity matrix and $^\chi$ indicates the skew-symmetric matrix. The state vector for the attitude of the spacecraft is ${\bm{x}} = [{\mathbf{q},\bm{\omega},\bm{\psi}}]^T$, and the control vector is ${\mathbf{u=\dot{\bm{\psi}}}} \in \mathbf{\mathcal{U}}$, and the dynamics are given by,
% \begin{equation}
%     \begin{bmatrix}
%         \dot{q}_1 \\ \dot{q}_2 \\ \dot{q}_3 \\ \dot{q}_4 \\ \dot{\omega}_1 \\ \dot{\omega}_2 \\ \dot{\omega}_3 \\ \dot{\psi}_1 \\ \dot{\psi}_2 \\ \dot{\psi}_3 
%     \end{bmatrix} = \begin{bmatrix}
%         \frac{1}{2}(q_4\omega_1-q_3\omega_2+q_2\omega_3) \\
%         \frac{1}{2}(q_3\omega_1+q_4\omega_2-q_1\omega_3) \\
%         \frac{1}{2}(-q_2\omega_1+q_1\omega_2+q_4\omega_3) \\
%         \frac{1}{2}(-q_1\omega_1-q_2\omega_2-q_3\omega_3) \\
%         J_1^{-1}((J_2-J_3)\omega_1\omega_3+D\dot{\psi}_1) \\ J_2^{-1}((J_3-J_1)\omega_2\omega_3+D\dot{\psi}_2) \\ J_3^{-1}((J_1-J_2)\omega_1\omega_2+D\dot{\psi}_3)\\ u_1 \\ u_2 \\ u_3        
%     \end{bmatrix}
% \end{equation}
% The values used for this work are $D=4.1\times10^-5\:kg-m^2, J_1 = 0.022\:kg-m^2, J_2 = 0.044\:kg-m^2,$ and $J_3 = 0.056\:kg-m^2$ \cite{petersen2021challenge}.
% \subsubsection{Translational}
% %CW Equations
% The position and velocity of the deputy relative to the chief in Hill's reference frame are denoted as ${\bm{r}}_H = x \hat{i}_H + y \hat{j}_H + z \hat{k}_H$ and ${\bm{v}}_H = \dot{x} \hat{i}_H + \dot{y} \hat{j}_H + \dot{z} \hat{k}_H$, respectively. The thrust applied by the deputy aligns with the body frame axis but can be represented in Hill's frame as ${\bm{u}}_T = F_x \hat{i}_H + F_y \hat{j}_H + F_z \hat{k}_H$. The Clohessy-Wiltshire equations \cite{clohessy1960terminal} provide a first-order approximation of the relative translational motion between the deputy and chief spacecraft as 
% \begin{equation}
% \begin{split}
%     \ddot{x} = 3n^2x+2n\dot{y}+F_x/m \\
%     \ddot{y} = -2n \dot{x} + F_y/m \\
%     \ddot{z} = -n^2 z +F_z/m
% \end{split}
% \end{equation}
% where $n$ is the spacecraft mean motion and $m$ is the mass of the deputy spacecraft. This work uses values of $n=0.001027\:rad/s$ and $m = 12\:kg$.
% \subsubsection{Temperature}
% The temperature of the spacecraft is modeled using thermal nodes, where each side of the spacecraft is represented by one node. For this analysis, it is assumed that each node is independent, and heat is not transferred between nodes. To determine the temperature of each node, four environmental heat fluxes are considered: solar flux, Earth albedo radiation, Earth Infared Radiation (IR), and heat rejection from the spacecraft \cite{foster2022small}. Solar flux, which is radiant energy from the sun, is the largest heat source for the spacecraft in LEO. The heat transfer, $\dot{q}$, from solar flux is given by,
% \begin{equation} \label{e:t_sol}
%     \dot{q}_{solar}=\alpha{}AS(\hat{n}\cdot \hat{r}_S)
% \end{equation}
% where $\alpha$ is the absorptivity of the surface, $A$ is the surface area, $S=1367\:W/m^2$ is the solar constant \cite{wertz1999space}, $\hat{n}$ is the surface normal vector, and $\hat{r}_S$ is the unit vector pointing from the surface to the sun. The sun incidence angle $\theta_{SI}$ is formed from $\hat{n}$ and $\hat{r}_S$ as shown in Figure \ref{f:sun_in}.
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=2in]{Figures/SunIncidence.png}
%     \caption{Sun Incidence Angle.}
%     \label{f:sun_in}
% \end{figure}
% Note that $\theta_{SI}$ is only defined on the interval $[0,\frac{\pi}{2}]$, and therefore $\dot{q}_{solar}=0$ when $\hat{n}\cdot \hat{r}_S \leq 0$.
% Earth albedo radiation is the solar energy that is reflected by the Earth, and is dependent on the conditions of the surface of the Earth. The transfer is given by, 
% \begin{equation}\label{e:t_albedo}
%     \dot{q}_{albedo}=\alpha A S A_f F_E
% \end{equation}
% where $A_f$ is the albedo factor of Earth, which is assumed to be $0.27$ \cite{wertz1999space}, and $F_E$ is the view factor between the surface and earth. Determination of the view factor for Earth can become complex \cite{garzon2018thermal}, but for this analysis it is simplified to $F_E=0.8\cos{\theta_{EI}}$ , where $\theta_{EI}$ is the incidence angle between the surface normal vector and the unit vector pointing from the surface to the Earth $\hat{r}_E$. In Hill's reference frame, the Earth always points along the $-\hat{x}$ axis, therefore $\hat{r}_E=[-1,0,0]^T$.
% Earth IR is heat emitted by the Earth, where the heat transfer is given by,
% \begin{equation}\label{e:t_ir}
%     \dot{q}_{IR}=\sigma \epsilon A F_E T_E^4
% \end{equation}
% where $\sigma=5.67051\times10^{-8}\:W/(m^2\times K^4)$ is the Stefan-Boltzmann constant \cite{wertz1999space}, $\epsilon$ is the surface emissivity, and $T_E$ is the temperature, which on average is $255\:K$ \cite{foster2022small}.
% Heat is rejected by the spacecraft into open space through radiation, where the heat transfer is given by,
% \begin{equation}\label{e:t_rej}
%     \dot{q}_{rejected} = \sigma \epsilon A T^4
% \end{equation}
% where $T$ is the temperature of the surface and the temperature of space is assumed to be zero. 
% The total heat transfer foe a node is then given by,
% \begin{equation}
%     \dot{q}_{total} = \dot{q}_{solar}+\dot{q}_{albedo}+\dot{q}_{IR}-\dot{q}_{rejected}
% \end{equation}
% The derivative of the temperature is then given by
% \begin{equation}
%     \dot{T}=\frac{\dot{q}_{total}}{mc_p}
% \end{equation}
% where $m$ is the mass of the node and $c_p$ is the specific heat of the material. For this paper, the temperature of one side of the spacecraft is tracked, which has $m=2\:kg$ and $A=300\:cm^2$. This side is assumed to be made of aluminum, which has the properties: $c_p=900\:J/(kg\times K)$, $\alpha=0.13$, and $\epsilon=0.06$ \cite{wertz1999space}.
% \subsubsection{Energy}
% For this simulation, the spacecraft has a battery and solar panels to charge the battery. In order to generate power, the solar panels must be facing the sun, where $\theta_{SI}\in [-\frac{\pi}{2},\frac{\pi}{2}]$. The power generated by the solar panels, $P_{in}$, is given by,
% \begin{equation}
%     P_{in} = P_I I_d A \cos{\theta_{SI}}
% \end{equation}
% where $P_I$ is the ideal performance and $I_d$ is the inherent degradation of the solar panels. The change in energy of the battery is given by,
% \begin{equation}
%     \dot{E}=P_{in}-P_{out}
% \end{equation}
% where the energy used by the spacecraft, $P_{out}$, is assumed to be a constant value of $15\:W$. The solar panels characteristics are: $P_I =983.3\:W$ \cite{bluePower} and $I_d=0.77$ \cite{wertz1999space}.
% \subsubsection{Sun}
% With the Earth and spacecraft fixed in Hill's reference frame, the sun is considered to rotate around the spacecraft. For this analysis, it is assumed that the sun rotates at a constant rate in the $\hat{x}-\hat{y}$ plane. The unit vector pointing from the center of the spacecraft to the sun, $\hat{r}_S$, is defined as,
% \begin{equation}
%     \hat{r}_S = [\cos{\theta_S},\cos{\theta_S},0]
% \end{equation}
% The change in angle $\theta_S$ is dependent on the spacecraft mean motion, $n$, such that $\dot{\theta}_S=-n$. In terms of angular rates, this is given by ${\bf{\omega}} = [0,0,-0.001027]^T$. Note, while the Sun is considered to move while the earth is stationary, it is assumed that the Earth never blocks sunlight from reaching the spacecraft. 
% \subsubsection{Total System Dynamics}
% Combining the dynamics formulated in the previous subsections, the full state vector of the system becomes ${\bm{x}} = [{\bf{q}},{\bm{\omega}},{\bm{\psi}},T,E,\theta_S,x,y,z,\dot{x},\dot{y},\dot{z}]^T$, and the control vector for the system is ${\bm{u}} = [{\bm{\psi}}, F_x, F_y, F_z]$. For the ASIF RTA, the functions $f({\bm{x}})$ and $g({\bm{x}})$, using the full state vector, are given by,
% \begin{equation} \label{e:full_dynamics}
% \begin{split}
%     f({\bm{x}})= \begin{bmatrix}
%         \frac{1}{2}(q_4\omega_1-q_3\omega_2+q_2\omega_3) \\
%         \frac{1}{2}(q_3\omega_1+q_4\omega_2-q_1\omega_3) \\
%         \frac{1}{2}(-q_2\omega_1+q_1\omega_2+q_4\omega_3) \\
%         \frac{1}{2}(-q_1\omega_1-q_2\omega_2-q_3\omega_3) \\
%         J_1^{-1}(J_2-J_3)\omega_1\omega_3 \\ J_2^{-1}(J_3-J_1)\omega_2\omega_3 \\ J_3^{-1}(J_1-J_2)\omega_1\omega_2\\ 0 \\ 0 \\ 0 \\ \dot{q}_{total}/(mc_p) \\ P_{in}-P_{out} \\ -n  \\
%         \dot{x}\\ \dot{y} \\ \dot{z} \\ 3n^2x+2n\dot{y} \\ -2n\dot{x}\\-n^2z
%     \end{bmatrix}, \\
%     g({\bm{x}}) = \begin{bmatrix}
%     0&0&0&0&0&0 \\ 0&0&0&0&0&0 \\ 0&0&0&0&0&0 \\ 0&0&0&0&0&0 \\ \frac{D}{J_1} &0&0&0&0&0\\ 0&\frac{D}{J_2} &0&0&0&0\\ 0&0& \frac{D}{J_3}&0&0&0\\
%     1&0&0&0&0&0 \\ 0&1&0&0&0&0 \\ 0&0&1&0&0&0 \\ 0&0&0&0&0&0 \\ 0&0&0&0&0&0 \\ 0&0&0&0&0&0 \\ 0&0&0&\frac{1}{m}&0&0\\ 0&0&0&0&\frac{1}{m}&0\\ 0&0&0&0&0&\frac{1}{m}
%     \end{bmatrix} \\
%     \end{split}
% \end{equation}
% \subsection{Constraints}\label{s:constraints}
% This section details the constraints on the spacecraft attitude and relative-motion. The constraints are derived from rotational and translational safety requirements that were generated from concerns of satellite operators and formally described in Reference \cite{hobbs2021risk}. The constraints are formatted as $h({\bm{x}})$ but implemented as BC as in Eq. \ref{e:BC}. The translational constraints (Safe Separation, Dynamic Speed, Passively Safe Maneuvers, and the translational velocity limits)  are a subset of the constraints developed in Reference \cite{dunlap2023run2}. This constraints are developed such that they are control invariant. Due to the complexity of the attitude dynamics and constraints, the attitude constraints only define the safe set and are not proven to be control invariant.
% % also reword this sentence to sound better, ARPOD paper has better explination of the constraints. should reference that and not go into as much detail here? 
% % Refenence Dunlap RTA for translational control for translatinal constraints?
% \subsubsection{Safe Separation} 
% The deputy spacecraft shall not collide with the chief. This constraint is defined as
% \begin{equation}
%     \phi_{col}({\bm{x}}) = ||{\bm{r_h}}||_2 - (r_d+r_c)
% \end{equation}
% where $r_d$ is the collision radius of the deputy and $r_c$ is the collision radius of the chief. From Reference \cite{dunlap2023run2}, it can be shown that this constraint is forward invariant when accounting for the need for the spacecraft to start slowing down to avoid a collision \cite{hibbard2022guaranteeing}. This constraint is then written as 
% \begin{equation}
%     h_{col}({\bm{x}}) = \sqrt{2a_max(||{\bm{r_h}}||_2-(r_d+r_c))}+{\bm{v_{hr}}}
% \end{equation}
% where ${\bm{v_{hr}}}$ is the projection of the deputy's velocity onto its position vector and $a_{max}$ is the worst-case acceleration due to natural motion from the system. This constraint only needs to be enforced when the deputy is moving towards the chief.
% \subsubsection{Dynamic Speed Constraint}
% The speed of the deputy shall decrease as it moves closer to the chief. This constraint reduces the risk of high speed collisions and ensures the deputy is moving slow enough to properly inspect the chief. The constraint is defined as,
% \begin{equation}
%     h_{speed}({\bm{x}}) = \nu_0+\nu_1||({\bm{r_H}})||_2-||({\bm{v}})||_2
% \end{equation}
% where $\nu_0$ is the minimum allowable speed, $\nu_1$ is the constant rate at which ${\bm{r_H}}$ shall decrease, and ${\bm{v}} =[\dot{x},\dot{y},\dot{z}]^T$. From Reference \cite{dunlap2021comparing}, it can be shown that as long as $u_{max}$ adheres to the following limit,
% \begin{equation}
%     \nu_1 \sqrt{3}v_{max}+3n^2\frac{\sqrt{3}v_{max}-\nu_0}{\nu_1}+2nv_{max} \leq \frac{u_{max}}{m},
% \end{equation}
% this constraint is control invariant.
% \subsubsection{Passively Safe Maneuvers}
% The deputy shall not collide with the chief in the event of thruster failure. This constraint ensures that if ${\bm u} =0$ then the resulting Free Flight Trajectory (FFT), ${\bm{r_H}}(t)$ will not intersect with the chief for all future time. The FFT is found by using a closed form solution of the Clohessy-Wiltshire equations \cite{dunlap2023run2}. The constraint is defined as,
% \begin{equation}
%     h_{pass} ({\bm{x}}) = \infin_{t\in[t_0,t_0+T]} ||{\bm{r_h}}(t)||_2 - (r_d+r_c)
% \end{equation}
% where $T$ is the time period to evaluate starting at $t_0$. This constraint is only guaranteed for all future time if $T=\infty$, but for implementation it is a finite value.
% \subsubsection{Attitude Exclusion Zone}
% The spacecraft shall adhere to conical attitude exclusion zones. For example, to avoid instrument blinding, it may be necessary to prevent a sensor from pointing directly towards the Sun. Consider the unit vectors pointing along the sensor boresight, $\hat{r}_B$, and from the center of the spacecraft to the exclusion zone, $\hat{r}_{EZ}$. The angle between these two unit vectors, $\theta_{EZ}$, is found using the dot product as shown in Figure \ref{f:koz}. 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=3in]{Figures/koz.png}
%     \caption{Attitude Exclusion Zone.}
%     \label{f:koz}
% \end{figure}

% The attitude exclusion zone is then defined as,
% \begin{equation}
%     h_{EZ}({\bm{x}}) = \theta_{EZ} - \frac{\alpha_{FOV}}{2}-\beta
% \end{equation}
% where $\alpha_{FOV}$ is the sensor's field of view and $\beta$ is a safety buffer. This constraint is relative degree 2. Therefore, HOCBFs are used to transform $h_{EZ}$ into a valid CBF with Eq. \ref{e:HOBC}. For this simulation, $\hat{r}_{EZ}=\hat{r}_S$, $\hat{r}_{B}=\hat{n}_x$, $\alpha_{FOV}=60\:deg$, and $\beta = 10\:deg$. 

% \subsubsection{Communication}
% The spacecraft shall maintain attitude requirements for communication with the ground station. Consider the unit vectors pointing along the transmitters boresight, $\hat{r}_B$, and from the center of the spacecraft to the ground station, $\hat{r}_{GS}$. The angle between these two unit vectors, $\theta_{GS}$, is found using the dot production, and is shown in Figure \ref{f:kiz}. 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=2.5in]{Figures/kiz.png}
%     \caption{Communication Angle.}
%     \label{f:kiz}
% \end{figure}

% The communication constraint is then defined as,
% \begin{equation}
%     h_{comm}({\bm{x}}) = \frac{\alpha_{FOV}}{2}-\theta_{GS}
% \end{equation}
% This constraint is relative degree 2; therefore, HOCBFs are used to transform $h_comm$ into a valid CBF with Eq. \ref{e:HOBC}. For this simulation, $\hat{r}_{EZ}=\hat{r}_S$, $\hat{r}_{B}=\hat{n}_x$, $\alpha_{FOV}=60\: deg$, and $\beta = 10\:deg$. For this simulation, $\hat{r}_{GS}=\hat{r}_E$, $\hat{r}_{B}=\hat{n}_y$, and $\alpha_{FOV}=180\: deg$.
% \subsubsection{Maintain Acceptable Temperature}
% The spacecraft shall maintain acceptable temperature of all components. For example, certain components of the spacecraft may overheat, in which case the spacecraft shall maneuver to rotate the component away from significant heat sources, typically the Sun. Given the temperature of a component, $T$, the temperature constraint is defined simply as,
% \begin{equation}
%     h_{temp}(\bm{x}) = T_{max}-T
% \end{equation}
% This constraint is relative degree 3 and could be enforced using HOCBFs; however, the Sun and Earth incidence angles with the surface are added to achieve better performance. The constraint is then given as,
% \begin{equation}
%     \Psi_{temp}({\bm{x}}) = T_{max}-T-\delta_0(\frac{\pi}{2}-\theta_{SI})-\delta_1(\frac{\pi}{2}-\theta_{EI})
% \end{equation}
% where $\delta_0$ and $\delta_1$ are constant coefficients that are tuned external to the QP and $T_{max}$ is the maximum allowable temperature. This constraint is relative degree 2, where HOCBFs are then used to transform $\Psi_{temp}$ into a valod CBF. Note that when $\theta_{SI} > 90\:deg$ and $\theta_{EI}>90 \:deg$, the gradient of the constraint is zero. However, in this case, temperature is decreasing and is not approaching $T_{max}$, so the CBF is valid. For this simulation, $T_{max}=10\: ^o C$ and $T$ is measured on the side of the spacecraft pointing along the $-y_B$ axis.
% \subsubsection{Maintain Battery Charge}
% The spacecraft shall maintain attitude requirements for sufficient power generation. For example, the spacecraft shall point its solar panels towards the sun to ensure the battery remains charged. Given the battery energy, $E$, the battery charge constraint is defined simply as,
% \begin{equation}
%     h_{batt}({\bm{x}}) = E-E_{min}
% \end{equation}
% where $E_{min}$ is the minimum allowable energy level, determined such that at this point the spacecraft would be able to maintain minimum function as determined by the mission. This constraint is relative degree 3. In this case, note that the gradient of the constraint is zero when the sun incidence angle with the side of spacecraft with the solar panels, $\theta_{SI}$, is greater than $90\:deg$. Therefore HOCBFs cannot be used to enforce this constraint. To account for this, $\theta_{SI}$ is added to the constraint, which is then given by,
% \begin{equation}
%     \Psi({\bm{x}}) = E-E_{min}-\delta_2\theta_{SI}
% \end{equation}
% This constraint is relative degree 2, where HCBFs are then used to transform it into a valid CBF. For this simulation, $E_{min}=1\:kJ$, and solar panels are assumed to cove the side of the spacecraft pointing along the $+z_B$ axis.
% \subsubsection{Avoid Actuation Saturation}
% The spacecraft actuation strategy shall conserve actuator use to prevent wear when possible. This constrain is not enforced with RTA, but rather is implemented as the admissible control set ${\mathcal{U}}$. For this simulation, $\dot{\psi}_{max}=181.3\:rad/s^2$ and ${\mathcal{U}}=[-\dot{\psi}_{max},\dot{\psi}_{max}]^3$.
% \subsubsection{Avoid Aggressive Maneuvering}
% The spacecraft shall maneuver below a threshold to prevent structural damage. For example, if the spacecraft rotates too quickly components might break. This constraint enforces limits on the translational velocities, $\dot{x},\dot{y},\dot{z}$, angular velocity, $\bm{\omega}$, and angular acceleration, $\dot{\bm{\omega}}$, as well as the reaction wheel velocity, $\bm{\phi}$. The constraints for velocities and reaction wheel velocity are defined as,
% \begin{equation}
%     h_{\omega}({\bm{x}})=\omega_{max}^2-\omega^2
% \end{equation}
% \begin{equation}
%     h_{\psi}({\bm{x}})=\psi_{max}^2-\psi^2
% \end{equation}
% \begin{equation} \label{vel_lim}
% \begin{split}
%     h_{\dot{x}}({\bm{x}})=v_{max}^2-\dot{x}^2\\
%     h_{\dot{y}}({\bm{x}})=v_{max}^2-\dot{y}^2\\
%     h_{\dot{z}}({\bm{x}})=v_{max}^2-\dot{z}^2
%     \end{split}
% \end{equation}
% From Reference \cite{dunlap2021comparing}, it can be shown that Eq. \ref{vel_lim} are control invariant if $u_{max}$ adheres to the following limits,
% \begin{equation}
% \begin{split}
%     3n^2r_{max}+2nv_{max}\leq \frac{u_{max}}{m}\\ 2nv_{max}\leq \frac{u_{max}}{m}\\ n^2r_{max}\leq \frac{u_{max}}{m}
%     \end{split}
% \end{equation}
% These constraints are relative degree 1 and are valid CBFs. Since the angular acceleration is not a state, it must be enforced differently. Given the system dynamics, $\dot{\omega}$ is directly related to $\dot{\phi}$ and $\omega$, so additional bounds for $\dot{\phi}_{max}$ can be used to enforce the constraint. The maximum angular acceleration occurs when ${\bm{\omega}} = [\omega_{max}]^3$ and  ${\dot{\bm{\omega}}} = [\dot{\omega}_{max}]^3$. From the system dynamics in Eq. \ref{e:full_dynamics}, enforcing the following constraints ensures that $|\dot{\omega}|\leq \dot{\omega}_{max}$,
% \begin{equation}
% \begin{split}
%     |\dot{\psi}_1| \leq \frac{J_1\dot{\omega}_{max} - |J_2-J_3|\omega_{max}^2}{D} \\
%     |\dot{\psi}_2| \leq \frac{J_2\dot{\omega}_{max} - |J_3-J_1|\omega_{max}^2}{D} \\
%     |\dot{\psi}_3| \leq \frac{J_3\dot{\omega}_{max} - |J_1-J_2|\omega_{max}^2}{D}
%     \end{split}
% \end{equation}
% These constraints are enforced as additional bounds on the admissible control set ${\mathcal{U}}$. For this simulation, $\dot{\omega}_{max} = 2\:deg/s^2$, $\omega_{max}=1\:deg/s$, and $\phi_{max}=576\:rad/s$.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Simulation Results}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This section presents the results of a simulation developed to test the constraints outlined in Section \ref{s:constraints}, where ASIF RTA is used to assure safety. This simulation uses the Safe Autonomy Run Time Assurance Framework \cite{ravaioli2023universal}, which simplifies user effort and supports automatic differentiation of all constraints, becoming particularly useful for the constraints that utilize HOCBFs.
% \subsection{Monte-Carlo Analysis}
% To verify that the RTA works regardless of initial conditions, a Monte-Carlo experiment was conducted. The simulations initialize random initial conditions that are within the safe set, such that no constraints are violated. To prevent a state being initialized on the constraint boundary, a $5\%$ buffer is added. 
% % DISCUSS QP FAILING AND WORK AROUNDS

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Conclusions}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % FUTURE WORK: IF JUST HAVE 3DOF THEN DISCUSS 6DOF AND ISSUES WITH MULTI-TIME SCALE DYNAMICS

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \appendices{}              % note there is no {} to put a title. Each appendix has its own title
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % For a single appendix, use the \appendix{} keyword and do not use the \section command.

% \section{More Information}        % first appendix
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% This is the first appendix. 

% \subsection{Comments}
% If you have only one appendix, use the ``appendix'' keyword.

% \subsection{More Comments}
% Use section and subsection keywords as usual.

% \section{Yet More Information}    % second appendix
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This is the second appendix.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \acknowledgments
% This work is supported by the Department of Defense through the Air Force Research Laboratory. The views expressed are those of the authors and do not reflect the official guidance or position of the United States Government, the Department of Defense or of the United States Air Force.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \bibliographystyle{IEEEtran}
% %\bibliography{IEEEabr,MyBibFile}
% \bibliography{references}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \thebiography
% %% This biostyle allows you to insert your photo size 1in X 1.25in
% \begin{biographywithpic}{Kerianne L. Hobbs}{Figures/HobbsKerianne8x10}
% is the Safe Autonomy and Space Lead on the Autonomy Capability Team (ACT3) at the Air Force Research Laboratory. There she investigates rigorous specification, analysis, bounding, and intervention techniques to enable safe, trusted, ethical, and certifiable autonomous and learning controllers for aircraft and spacecraft applications. Her previous experience includes work in automatic collision avoidance and autonomy verification and validation research. Dr. Hobbs was selected for the 2020 AFCEA 40 Under 40 award and was a member of the team that won the 2018 Collier Trophy (Automatic Ground Collision Avoidance System Team), as well as numerous AFRL Awards.  Dr. Hobbs has a BS in Aerospace Engineering from Embry-Riddle Aeronautical University, an MS in Astronautical Engineering from the Air Force Institute of Technology, and a Ph.D. in Aerospace Engineering from the Georgia Institute of Technology. 
% \end{biographywithpic}




% \end{document}

==> Main_obs_attitude.tex <==
% % % IEEEAerospace2012.cls requires the following packages: times, rawfonts, oldfont, geometry
% % \documentclass[twocolumn,letterpaper]{IEEEAerospaceCLS}  % only supports two-column, letterpaper format

% % % The next line gives some packages you may find useful for your paper--these are not required though.
% % %\usepackage[]{graphicx,float,latexsym,amssymb,amsfonts,amsmath,amstext,times,psfig}
% % % NOTE: The .cls file is now compatible with amsmath!!!

% % \usepackage[]{graphicx}    % We use this package in this document
% \usepackage{amsfonts}
% \newcommand{\ignore}[1]{}  % {} empty inside = %% comment

% \usepackage{xurl} % allows break in url so it doesnt run into next column
% \usepackage{amsmath}
% \DeclareMathOperator*{\argmin}{argmin} % thin space, limits underneath in displays
% \usepackage{amsmath,amsfonts,amsthm,bm} % Math packages


% \begin{document}
% \title{Run Time Assured Reinforcement Learning for Spacecraft Attitude Maneuvering}

% \author{
% Cassie-Kay McQuinn\\ 
% Department of Aerospace Engineering\\
% Texas A\&M University\\
% College Station, TX, 77843\\
% ckmcquinn@tamu.edu
% \and 
% Kyle Dunlap\\
% Parallax Advanced Research\\
% 4035 Colonel Glenn Hwy\\
% Beavercreek, OH, 45431 \\
% kyle.dunlap@parallaxresearch.org
% \and 
% Nathaniel Hamilton\\
% Parallax Advanced Research\\
% 4035 Colonel Glenn Hwy\\
% Beavercreek, OH, 45431 \\
% nathaniel.hamilton@parallaxresearch.org
% \and
% Jabari Wilson\\
% Department of Mechanical Engineering\\
% University of Florida\\
% Gainesville, Florida, 32611\\
% jabari.wilson@outlook.com
% \and
% Kerianne L. Hobbs\\ 
% Air Force Research Laboratory\\
% 2241 Avionics Circle\\
% Wright-Patterson AFB, OH, 45433\\
% kerianne.hobbs@us.af.mil
% %%%% IMPORTANT: Use the correct copyright information--IEEE, Crown, or U.S. government. %%%%%
% \thanks{\footnotesize 979-8-3503-0462-6/24/$\$31.00$ \copyright2024 IEEE}              % This creates the copyright info that is the correct 2024 data.
% %\thanks{{U.S. Government work not protected by U.S. copyright}}         % Use this copyright notice only if you are employed by the U.S. Government.
% %\thanks{{979-8-3503-0462-6/24/$\$31.00$ \copyright2024 Crown}}          % Use this copyright notice only if you are employed by a crown government (e.g., Canada, UK, Australia).
% %\thanks{{979-8-3503-0462-6/24/$\$31.00$ \copyright2024 European Union}}    % Use this copyright notice is you are employed by the European Union.
% }



% \maketitle

% \thispagestyle{plain}
% \pagestyle{plain}



% \maketitle

% \thispagestyle{plain}
% \pagestyle{plain}

% \begin{abstract}

%  A fundamental capability for On-orbit Servicing, Assembly, and Manufacturing (OSAM) is inspection of the vehicle to be serviced, or the structure being assembled. This research investigates autonomous slewing to maintain situational awareness of multiple vehicles operating in close proximity where several safety constraints must be satisfied. A reinforcement learning solution is used as a primary controller to command slewing. Run time assurance (RTA) monitors system behavior and the output of the neural network control system trained using reinforcement learning to enforce safety constraint satisfaction during training as well as during testing. This research explores combining a subset of the constraints into an Active Set Invariance Filter (ASIF) RTA defined using control barrier functions that is minimally invasive to the primary control, by minimizing deviation from the desired control output of the neural network control system, while simultaneously enforcing all safety constraints. The RTA is designed to ensure the spacecraft maintains attitude requirements for communication and data transfer with a ground station during scheduled communication windows, adheres to conical attitude keep out zones, limits thermally unfavorable attitude duration, maintains attitude requirements for sufficient power generation, ensures maneuvers are below threshold to cause structural damage, ensures maximum angular velocity is below limits to maintain ability to respond quickly to new slewing commands, and conserves actuator use to prevent wear when possible. Simulation results are shown and evaluated for a three degree of freedom spacecraft with reaction wheel attitude control. 

% \end{abstract} 


% \tableofcontents

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Introduction}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % discuss background of safe RL, RTA. Why its important and what has currently been done. Previous work has satisfied one control barrier function but this work aims to satisfy multiple as well as priority rank?
% % background on mission - Vehicle inspection 
% % On-orbit Servicing Assembly and Manufacturing (OSAM) 
% % why do we care about RL

% % OSAM source? can include example of OSAM such as ISS, Hubble telescope, and Mission Extension Vehicles

% % this is only those registered with UNOOS, need a way to say that there are likely more
% According to the United Nation's Register of Objects Launched into Outer Space \cite{OSOidx}, 2474 registered objects were launched into outer space in 2022. Comparing this to the 222 registered objects that were launched in 2015, the space industry is growing at a rapid pace. With this growth comes a change in the manner with which missions are conducted, introducing a paradigm shift with the emerging technology of On-orbit Servicing, Assembly, and Manufacturing (OSAM) \cite{arney2021orbit}. OSAM will facilitate extended space missions, orbital manipulation of existing objects, such as the removal of space debris, and repair of existing satellite systems. A major capability of OSAM is the inspection task. Inspection is the observation of systems to analyze features of interest, including damaged assets or assembly of new  components. Inspection vehicles must maintain situational awareness of multiple vehicles operating in close proximity. Additionally, safety and mission constraints on the inspection vehicle must be satisfied for the vehicle to successfully complete the inspection task. \\
% A safe set of states are formed where all the constraints. Due to the multiple constraints deriving a controller that keeps the spacecraft within the set for all time using traditional control techniques. Through trail-and-error search, Reinforcement Learning (RL) determines, or \textit{learns}, which actions maximize a reward \cite{sutton2018reinforcement}. For autonomous spacecraft operations, this enables high performance for low online computational complexity. In RL, training occurs offline during the design phase, then a 


% Building off of the work in by Dunlap et al. \cite{dunlap2023run}, this research will utilize Run Time Assurance (RTA) during RL training in order to enforce assurance to safety constraints. 

% investigate training with ASIF RTA due to the complexity of the constraints, it would be very difficult to determine a backup control law that satisfies all constraints.


% % other approches to solving this problem 
% % SOMETHING ABOUT DERVING A CONTROLLER BEING DIFFICULT BECAUSE OF ALL THE REQUIREMENTSadmin/manage/my-submissions
% % something about need for autonomy, can incorporate RL controller here

% The concept of safety....

% %"The concept of safety is fundamentally linked to the idea of constrained behavior" -ASIF paper


% % something about requirements of a system being satisfied, can incorporate need for RTA here

% % sentance about this work will 



% % why do we care about RTA
% % discuss the 4 main types of RTA systems here or in RTA section?
% % specify that its explicit RTA, why explicit rather than implicit?
% The contribution of this paper is the application of ASIF RTA, in training and testing, to enforce multiple safety constraints to a spacecraft with attitude control. The neural network is trained with ASIF RTA active to prevent the system from entering unsafe states. Then the controller is simulated on the spacecraft with ASIF RTA active to ensure adheres to the safety constraints. 

% % key points:
% % safety - RTA
% % RL controller
% % 
% This paper is organized as follows: 
% % Section 2: RTA
% % somewhere need to incorporate slack variables/constraint prioritization
% % Section 3: RL
% % Section 3: Spacecraft attitude representation/Methodology
% % Section 4: Simulation Results
% % Section 5: Conclusions
 


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Run Time Assurance}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This work considers a continuous-time control affine system defined as
% \begin{equation}\label{e:dynamics}
%     {\mathbf{\dot{x}}}=  f({\bm{x}})+ g({\bm{x}}){\bm{u}}
% \end{equation}
% where $\bm{x} \in \mathcal{X} \subseteq $ ${\mathbb{R}} ^ {n}$  denotes the state vector, ${\bm{u}} \in {\mathcal{U}} \subseteq {\mathbb{R}}^{m}$ denotes the control vector, and $f : \mathcal{X} \rightarrow  $ ${\mathbb{R}} ^ {n}$  and $g : \mathcal{X} \rightarrow $ ${\mathbb{R}} ^ {n \times m}$  are locally Lipschitz continuous functions. Here, $\mathcal{X}$ is the set of all possible state values and $\mathcal{U}$ is the admissible control set.\\
% RTA is an online safety assurance technique that filters the control inputs from a primary controller to preserve safety of the system. RTA filters are decoupled from the primary controller. This enabled the objective of the primary controller be to achieve the highest performance while the objective of the RTA filter is to assure safety. The RTA filter intercepts the desired control $\bm{u}_{des}$ from the primary controller, modifies it as necessary to assure safety, and then passes a new action $\bm{u}_{act}$ to the plant. A feedback control system with RTA is shown in figure \ref{rta_cl}.\\
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=3.25in]{Figures/RTAcontrolLoop.png}
%     \caption{Control Loop with RTA}
%     \label{rta_cl}
% \end{figure}
% The Active Set Invariance Filter (ASIF) RTA \cite{gurriet2018online} is an optimization-based technique designed to be minimally invasive towards the primary controller. ASIF algorithms use Control Barrier Functions (CBF) \cite{ames2019control} to enforce adherence to safety constraints. The ASIF algorithm used in this work is defined as
% \begin{equation}\label{e:ASIF}
%     \begin{gathered}
%     {\bm{u}}_{act}({\bm{x}},{\bm{u}}_{des}) = \argmin_{{\bm{u}} \in \mathcal{U}} \lvert \lvert {\bm{u}}_{des} - {\bm{u}} \rvert \rvert ^2 \\
%      \text{s.t. } BC_i({\bm{x}}, {\bm{u}}) \geq 0, \forall i\in \{1,..., M \} 
%     \end{gathered}
% \end{equation}
% ASIF uses a Quadratic Program (QP) to minimize the $l^2$ norm difference between ${\bm{u}}_{des}$ and ${\bm{u}}_{act}$, and therefore only modifies ${\bm{u}}_{des}$ when necessary to assure safety. The inequality constraint for the QP are a set of $M$ Barrier Constraints (BC). To define safety of the system, consider a set of $M$ continuously differentiable functions $h_i : {\mathcal{X}} \rightarrow {\mathbb{R}}, \forall i \in \{1,...,M\}$, then the safe set, $\mathcal{C}_S$, can be defined as,
% \begin{equation}
%     {\mathcal{C}}_S := \{ {\bm{x}} \in {\mathcal{X}} \lvert h_i({\bm{x}}) \geq 0, \forall i \in \{1,...,M \}.
% \end{equation}
% Note, this work focuses on safety defined explicitly rather than implicitly. Explicit safe sets are defined offline. Implicit safe sets are determined by evaluating trajectories using a predefined backup control law to evaluate if a given input will result in the system leaving the safe set. The system is considered safe if $\mathcal{C}_S$ is forward invariant with respect to Eq. \ref{e:dynamics}, such that, 
% \begin{equation}
%     {\bm{x}} ({t}_0) \in  {\mathcal{C}}_S \Rightarrow {\bm{x} }(t) \in{} {\mathcal{C}}_S , \forall{} \geq{} t_0.
% \end{equation}
% Barrier constraints, which are satisfied when $BC_i({\bm{x}},{\bm{u}}) \geq 0$, enforce Nagumo's condition \cite{nagumo1942lage}.
% The boundary of the set is formed by $h_i(\bm{x})$ and, if $\dot{h}_i(\bm{x})$ is never decreasing, then $\bm{x}$ will never leave the safe set ${\mathcal{C}}_S$. Since the boundary of a set does not have volume, a strengthening class-$\kappa$ infinity function, $\alpha$, is utilized to enforce the boundary condition. The resulting BC is defined as,
% \begin{equation}
%     BC({\bm{x}},{\bm{u}}) = \dot{h}({\bm{x}},{\bm{u}})+\alpha (h({\bm{x}}))
% \end{equation}
% where $\dot{h}({\bm{x}})$ is defined as,
% \begin{equation}
%     \dot{h}({\bm{x}})=\nabla h({\bm{x}})\dot{{\bm{x}}} = L_f h({\bm{x}})+L_g h({\bm{x}}) {\bm{u}} \geq 0,
% \end{equation}
% where $L_f$ and $L_g$ are Lie derivatives of $h_i$ along $f$ and $g$ respectively. Using Eq. \ref{e:dynamics}, the BC becomes,
% \begin{equation}\label{e:BC}
%     BC({\bm{x}},{\bm{u}}):=\nabla h({\bm{x}})(f({\bm{x}})+ g({\bm{x}}){\bm{u}}) + \alpha (h({\bm{x}}))
% \end{equation}
% \subsection{High Order Control Barrier Functions}
% For some constraints, $\nabla h({\bm{x}})$ may not depend on the control input. In this case, the BC is not valid as $\nabla h({\bm{x}})g({\bm{x}}){\bm{u}}=0$. To solve this problem, High Order Control Barrier Functions (HOCBF) can be used to differentiate the constraint and allow $\nabla h({\bm{x}})$ to depend on $\bm{u}$. A sequence of functions ${{\Psi}}_j: {\mathbb{R}}^n \rightarrow {\mathbb{R}}, \forall j \in \{1,...,m\}$ is defined as,
% \begin{equation}\label{e:HOBC}
%     {{\Psi}}_j({\bm{x}}):=\dot{{{\Psi}}}_{j-1}({\bm{x}}) + \alpha_j({{\Psi}}_j({\bm{x}})), \forall j \in \{1,...,m\},
% \end{equation}
% where $m$ us referred to as the relative degree of the system and is the number of times needed to differentiate the constraint in order for the control to explicitly appear in the corresponding derivative \cite{xiao2022control}. In this case, $\Psi_0({\bm{x}}) = h({\bm{x}})$ and $\dot{\Psi}({\bm{x}})g({\bm{x}}) \neq 0$. In the cases where $j<m, \dot{\Psi}({\bm{x}}))=\nabla\Psi({\bm{x}})f({\bm{x}})$. Also note that when $m=1, \Psi({\bm{x}})$ is equivalent to Eq. \ref{e:BC}.
% \subsection{Slack Variables}
% When simulating a system with multiple safety constraints, there can be situations or conditions in which these constraints conflict with each other. This will cause the QP to fail if it can not find a solution without violating a constraint. In order to prevent this from occurring, a slack variable $\delta$ can be added into Eq. \ref{e:ASIF} such that it becomes 
% \begin{equation}\label{e:ASIF_slack}
%     \begin{gathered}
%     {\bm{u}}_{act}({\bm{x}},{\bm{u}}_{des}) = \argmin_{{\bm{u}},\delta \in \mathcal{U}} \lvert \lvert {\bm{u}}_{des} - {\bm{u}} \rvert \rvert ^2 + \sum_ip_i\delta_i^2 \\
%      \text{s.t. } BC_i({\bm{x}}, {\bm{u}}) \geq \delta_i, \forall i\in \{1,..., M \} 
%     \end{gathered}
% \end{equation}
% The QP also solves for the slack variables which adds a buffer on the constraint. $p$ is a hyper-parameter that correlates to a scaling constant on the slack variable. Its value should be large (for example $10^{12}$) such that the slack variable is only non zero in the case that the QP cannot be solved. For the QP to have a unique solution, there can be $M-1$ slack variables, meaning at least one constraint cannot have a slack variable. Including slack variables relaxes the constraint, so it should only be included on constraints that can be violated or the lowest priority constraints.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Reinforcement Learning Control Law}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Problem Formulation}\label{s:pf}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The following sections describe the dynamics of the system and the constraints that are used to enforce safety. 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=2.5in]{Figures/cubeSat.png}
%     \caption{Hypothetical Cubesat.}
%     \label{f:cube_sat}
% \end{figure}
% \subsection{Dynamics}
% The spacecraft is modeled as a 6U CubeSat as shown in Figure \ref{f:cube_sat} with the body reference frame $(x_B,y_B,z_B)$. The spacecraft has an antenna on the $+y_B$ face for communication with a ground station, an arbitrary sensor on the $+x_B$ face, and a solar panel on the $+z_B$ face. The system dynamics are represented in Hill's reference frame \cite{hill1878researches} with the origin $O_H$ centered on the spacecraft in a circular orbit around Earth. As shown in Figure \ref{f:hill_frame}, the unit vector $\hat{x}$ points from the center of the spacecraft away from the center of the Earth, $\hat{y}$ points in the direction of motion of the spacecraft, $\vec{v}$, around the Earth, and $\hat{z}$ is normal to $\hat{x}$ and $\hat{y}$. For this problem, the spacecraft is assumed to remain in the same circular orbit in Low Earth Orbit (LEO) and it can only control its orientation via a three wheel reaction wheel array, where the reaction wheels are aligned with the principal. 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=3.25in]{Figures/HillsFrame.png}
%     \caption{Hill's Reference Frame.}
%     \label{f:hill_frame}
% \end{figure}
% This subsection outlines the dynamical models used for the attitude, surface temperature, and stored energy of the spacecraft as well as the dynamics for the sun in the simulation.
% \subsubsection{Attitude}
% The attitude of the spacecraft is modeled in the principal axis body reference frame, where the origin is located at the center of mass of the spacecraft, and the axes are aligned with the eigenvectors of the spacecraft inertia matrix. The attitude is then modeled using a quaternion formulation \cite{markley2014fundamentals}, which represents a rotation between two reference frames. In this case, the quaternion is used to represent the rotation of the spacecraft from Hill's reference frame to the body reference frame. The quaternion also avoids singularity points that arise from Euler angles. A quaternion ${\mathbf{q}} \in {\mathbb{R}}^4$ is comprised of a three vector part ${\mathbf{q}}_v= {\mathbf{q}}_{1:3}$ and a scalar part $q_4$. The angular rates ${\bm{\omega}} \in {\mathbb{R}}^3$ are then used to represent the rotation of the spacecraft about each of its principal axes. The derivative of the angular rates is given by Euler's rotation equations,
% \begin{equation}\label{e:eulerRot}
%     {\mathbf{J}\dot{\bm{\omega}}+\bm{\omega} \times \bf{J}\bm{\omega} = \bm{\tau}},
% \end{equation}
% where $\mathbf{J}$ is the spacecraft's inertia matrix and $\bm{\tau}$ is the torque applied to the spacecraft via the reaction wheels. Therefore, ${\bm{\tau}} = D{\dot{\bm{\psi}}}$, where $D$ is the reaction wheel spin axis mass moment of inertia and ${\dot{\bm{\psi}}}$ is the reaction wheel acceleration. Eq. \ref{e:eulerRot} can then be written in the principal axis body reference frame as,
% \begin{equation}
%     \begin{bmatrix} 
%         \dot{\omega}_1 \\ \dot{\omega}_2 \\ \dot{\omega}_3
%     \end{bmatrix} =
%     \begin{bmatrix}
%         J_1^{-1}((J_2-J_3)\omega_1\omega_3+D\dot{\psi}_1) \\ J_2^{-1}((J_3-J_1)\omega_2\omega_3+D\dot{\psi}_2) \\ J_3^{-1}((J_1-J_2)\omega_1\omega_2+D\dot{\psi}_3)
%     \end{bmatrix}
% \end{equation}
% Here, $J_1,J_2,$ and $J_3$ are the principal moments of inertia of the spacecraft. The relation of the quaternion derivatives to the angular rates is given by,
% \begin{equation}
%     {\mathbf{\dot{q}}} = \frac{1}{2}{\mathbf{\Xi}}(\mathbf{q})\bm{\omega}
% \end{equation}
% where $\mathbf{\Xi}$ is given by,
% \begin{equation}
%     {\mathbf{\Xi}}({\mathbf{q}})=\begin{bmatrix}
%         q_s{\mathcal{I}}-{\mathbf{q}}_v^\chi \\ -{\mathbf{q}}_v^T
%     \end{bmatrix} = \begin{bmatrix}
%         q_4 & -q_3 & q_2 \\ q_3 & q_4 & -q_1 \\ -q_2 & q_1 & q_4 \\ -q_1 & -q_2 & -q_3
%     \end{bmatrix}
% \end{equation}
% where ${\mathcal{I}} \in {\mathbb{R}}^3$ represents the identity matrix and $^\chi$ indicates the skew-symmetric matrix. The state vector for the attitude of the spacecraft is ${\bm{x}} = [{\mathbf{q},\bm{\omega},\bm{\psi}}]^T$, and the control vector is ${\mathbf{u=\dot{\bm{\psi}}}} \in \mathbf{\mathcal{U}}$, and the dynamics are given by,
% \begin{equation}
%     \begin{bmatrix}
%         \dot{q}_1 \\ \dot{q}_2 \\ \dot{q}_3 \\ \dot{q}_4 \\ \dot{\omega}_1 \\ \dot{\omega}_2 \\ \dot{\omega}_3 \\ \dot{\psi}_1 \\ \dot{\psi}_2 \\ \dot{\psi}_3 
%     \end{bmatrix} = \begin{bmatrix}
%         \frac{1}{2}(q_4\omega_1-q_3\omega_2+q_2\omega_3) \\
%         \frac{1}{2}(q_3\omega_1+q_4\omega_2-q_1\omega_3) \\
%         \frac{1}{2}(-q_2\omega_1+q_1\omega_2+q_4\omega_3) \\
%         \frac{1}{2}(-q_1\omega_1-q_2\omega_2-q_3\omega_3) \\
%         J_1^{-1}((J_2-J_3)\omega_1\omega_3+D\dot{\psi}_1) \\ J_2^{-1}((J_3-J_1)\omega_2\omega_3+D\dot{\psi}_2) \\ J_3^{-1}((J_1-J_2)\omega_1\omega_2+D\dot{\psi}_3)\\ u_1 \\ u_2 \\ u_3        
%     \end{bmatrix}
% \end{equation}
% The values used for this work are $D=4.1\times10^-5\:kg-m^2, J_1 = 0.022\:kg-m^2, J_2 = 0.044\:kg-m^2,$ and $J_3 = 0.056\:kg-m^2$ \cite{petersen2021challenge}.
% \subsubsection{Temperature}
% The temperature of the spacecraft is modeled using thermal nodes, where each side of the spacecraft is represented by one node. For this analysis, it is assumed that each node is independent, and heat is not transferred between nodes. To determine the temperature of each node, four environmental heat fluxes are considered: solar flux, Earth albedo radiation, Earth Infared Radiation (IR), and heat rejection from the spacecraft \cite{foster2022small}. Solar flux, which is radiant energy from the sun, is the largest heat source for the spacecraft in LEO. The heat transfer, $\dot{q}$, from solar flux is given by,
% \begin{equation} \label{e:t_sol}
%     \dot{q}_{solar}=\alpha{}AS(\hat{n}\cdot \hat{r}_S)
% \end{equation}
% where $\alpha$ is the absorptivity of the surface, $A$ is the surface area, $S=1367\:W/m^2$ is the solar constant \cite{wertz1999space}, $\hat{n}$ is the surface normal vector, and $\hat{r}_S$ is the unit vector pointing from the surface to the sun. The sun incidence angle $\theta_{SI}$ is formed from $\hat{n}$ and $\hat{r}_S$ as shown in Figure \ref{f:sun_in}.
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=2in]{Figures/SunIncidence.png}
%     \caption{Sun Incidence Angle.}
%     \label{f:sun_in}
% \end{figure}
% Note that $\theta_{SI}$ is only defined on the interval $[0,\frac{\pi}{2}]$, and therefore $\dot{q}_{solar}=0$ when $\hat{n}\cdot \hat{r}_S \leq 0$.
% Earth albedo radiation is the solar energy that is reflected by the Earth, and is dependent on the conditions of the surface of the Earth. The transfer is given by, 
% \begin{equation}\label{e:t_albedo}
%     \dot{q}_{albedo}=\alpha A S A_f F_E
% \end{equation}
% where $A_f$ is the albedo factor of Earth, which is assumed to be $0.27$ \cite{wertz1999space}, and $F_E$ is the view factor between the surface and earth. Determination of the view factor for Earth can become complex \cite{garzon2018thermal}, but for this analysis it is simplified to $F_E=0.8\cos{\theta_{EI}}$ , where $\theta_{EI}$ is the incidence angle between the surface normal vector and the unit vector pointing from the surface to the Earth $\hat{r}_E$. In Hill's reference frame, the Earth always points along the $-\hat{x}$ axis, therefore $\hat{r}_E=[-1,0,0]^T$.
% Earth IR is heat emitted by the Earth, where the heat transfer is given by,
% \begin{equation}\label{e:t_ir}
%     \dot{q}_{IR}=\sigma \epsilon A F_E T_E^4
% \end{equation}
% where $\sigma=5.67051\times10^{-8}\:W/(m^2\times K^4)$ is the Stefan-Boltzmann constant \cite{wertz1999space}, $\epsilon$ is the surface emissivity, and $T_E$ is the temperature, which on average is $255\:K$ \cite{foster2022small}.
% Heat is rejected by the spacecraft into open space through radiation, where the heat transfer is given by,
% \begin{equation}\label{e:t_rej}
%     \dot{q}_{rejected} = \sigma \epsilon A T^4
% \end{equation}
% where $T$ is the temperature of the surface and the temperature of space is assumed to be zero. 
% The total heat transfer foe a node is then given by,
% \begin{equation}
%     \dot{q}_{total} = \dot{q}_{solar}+\dot{q}_{albedo}+\dot{q}_{IR}-\dot{q}_{rejected}
% \end{equation}
% The derivative of the temperature is then given by
% \begin{equation}
%     \dot{T}=\frac{\dot{q}_{total}}{mc_p}
% \end{equation}
% where $m$ is the mass of the node and $c_p$ is the specific heat of the material. For this paper, the temperature of one side of the spacecraft is tracked, which has $m=2\:kg$ and $A=300\:cm^2$. This side is assumed to be made of aluminum, which has the properties: $c_p=900\:J/(kg\times K)$, $\alpha=0.13$, and $\epsilon=0.06$ \cite{wertz1999space}.
% \subsubsection{Energy}
% For this simulation, the spacecraft has a battery and solar panels to charge the battery. In order to generate power, the solar panels must be facing the sun, where $\theta_{SI}\in [-\frac{\pi}{2},\frac{\pi}{2}]$. The power generated by the solar panels, $P_{in}$, is given by,
% \begin{equation}
%     P_{in} = P_I I_d A \cos{\theta_{SI}}
% \end{equation}
% where $P_I$ is the ideal performance and $I_d$ is the inherent degradation of the solar panels. The change in energy of the battery is given by,
% \begin{equation}
%     \dot{E}=P_{in}-P_{out}
% \end{equation}
% where the energy used by the spacecraft, $P_{out}$, is assumed to be a constant value of $15\:W$. The solar panels characteristics are: $P_I =983.3\:W$ \cite{bluePower} and $I_d=0.77$ \cite{wertz1999space}.
% \subsubsection{Sun}
% With the Earth and spacecraft fixed in Hill's reference frame, the sun is considered to rotate around the spacecraft. For this analysis, it is assumed that the sun rotates at a constant rate in the $\hat{x}-\hat{y}$ plane. The unit vector pointing from the center of the spacecraft to the sun, $\hat{r}_S$, is defined as,
% \begin{equation}
%     \hat{r}_S = [\cos{\theta_S},\cos{\theta_S},0]
% \end{equation}
% The change in angle $\theta_S$ is dependent on the spacecraft mean motion, $n$, such that $\dot{\theta}_S=-n=-0.001027\:rad/s$. In terms of angular rates, this is given by ${\bf{\omega}} = [0,0,-0.001027]^T$. Note, while the Sun is considered to move while the earth is stationary, it is assumed that the Earth never blocks sunlight from reaching the spacecraft. 
% \subsubsection{Total System Dynamics}
% Combining the dynamics formulated in the previous subsections, the full state vector of the system becomes: ${\bm{x}} = [{\bf{q}},{\bm{\omega}},{\bm{\psi}},T,E,\theta_S]^T$. For the ASIF RTA, the functions $f({\bm{x}})$ and $g({\bm{x}})$, using the full state vector, are given by,
% \begin{equation} \label{e:full_dynamics}
% \begin{split}
%     f({\bm{x}})= \begin{bmatrix}
%         \frac{1}{2}(q_4\omega_1-q_3\omega_2+q_2\omega_3) \\
%         \frac{1}{2}(q_3\omega_1+q_4\omega_2-q_1\omega_3) \\
%         \frac{1}{2}(-q_2\omega_1+q_1\omega_2+q_4\omega_3) \\
%         \frac{1}{2}(-q_1\omega_1-q_2\omega_2-q_3\omega_3) \\
%         J_1^{-1}(J_2-J_3)\omega_1\omega_3 \\ J_2^{-1}(J_3-J_1)\omega_2\omega_3 \\ J_3^{-1}(J_1-J_2)\omega_1\omega_2\\ 0 \\ 0 \\ 0 \\ \dot{q}_{total}/(mc_p) \\ P_{in}-P_{out} \\ -n        
%     \end{bmatrix}, \\
%     g({\bm{x}}) = \begin{bmatrix}
%     0&0&0 \\ 0&0&0 \\ 0&0&0 \\ 0&0&0 \\ D/J_1 &0&0\\ 0&D/J_2 &0\\ 0&0& D/J_3\\
%     1&0&0 \\ 0&1&0 \\ 0&0&1 \\ 0&0&0 \\ 0&0&0 \\ 0&0&0
%     \end{bmatrix}
%     \end{split}
% \end{equation}
% \subsection{Constraints}\label{s:constraints}
% This section details the constraints on the spacecraft attitude. The constraints are derived from rotational safety requirements that were generated from concerns of satellite operators and formally described by Hobbs, et al. in \cite{hobbs2021risk}. The constraints are formatted as, $h({\bm{x}})$ but implemented as BC as in Eq. \ref{e:BC} or Eq. \ref{e:HOBC}.
% % also reword this sentence to sound better, ARPOD paper has better explination of the constraints. should reference that and not go into as much detail here? unsure of it was published
% \subsubsection{Attitude Exclusion Zone}
% The spacecraft shall adhere to conical attitude exclusion zones. For example, to avoid instrument blinding, it may be necessary to prevent a sensor from pointing directly towards the Sun. Consider the unit vectors pointing along the sensor boresight, $\hat{r}_B$, and from the center of the spacecraft to the exclusion zone, $\hat{r}_{EZ}$. The angle between these two unit vectors, $\theta_{EZ}$, is found using the dot product as shown in Figure \ref{f:koz}. 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=3in]{Figures/koz.png}
%     \caption{Attitude Exclusion Zone.}
%     \label{f:koz}
% \end{figure}

% The attitude exclusion zone is then defined as,
% \begin{equation}
%     h_{EZ}({\bm{x}}) = \theta_{EZ} - \frac{\alpha_{FOV}}{2}-\beta
% \end{equation}
% where $\alpha_{FOV}$ is the sensor's field of view and $\beta$ is a safety buffer. This constraint is relative degree 2. Therefore, HOCBFs are used to transform $h_{EZ}$ into a valid CBF with Eq. \ref{e:HOBC}. For this simulation, $\hat{r}_{EZ}=\hat{r}_S$, $\hat{r}_{B}=\hat{n}_x$, $\alpha_{FOV}=60\:deg$, and $\beta = 10\:deg$. 

% \subsubsection{Communication}
% The spacecraft shall maintain attitude requirements for communication with the ground station. Consider the unit vectors pointing along the transmitters boresight, $\hat{r}_B$, and from the center of the spacecraft to the ground station, $\hat{r}_{GS}$. The angle between these two unit vectors, $\theta_{GS}$, is found using the dot production, and is shown in Figure \ref{f:kiz}. 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=2.5in]{Figures/kiz.png}
%     \caption{Communication Angle.}
%     \label{f:kiz}
% \end{figure}

% The communication constraint is then defined as,
% \begin{equation}
%     h_{comm}({\bm{x}}) = \frac{\alpha_{FOV}}{2}-\theta_{GS}
% \end{equation}
% This constraint is relative degree 2; therefore, HOCBFs are used to transform $h_comm$ into a valid CBF with Eq. \ref{e:HOBC}. For this simulation, $\hat{r}_{EZ}=\hat{r}_S$, $\hat{r}_{B}=\hat{n}_x$, $\alpha_{FOV}=60\: deg$, and $\beta = 10\:deg$. For this simulation, $\hat{r}_{GS}=\hat{r}_E$, $\hat{r}_{B}=\hat{n}_y$, and $\alpha_{FOV}=180\: deg$.
% \subsubsection{Maintain Acceptable Temperature}
% The spacecraft shall maintain acceptable temperature of all components. For example, certain components of the spacecraft may overheat, in which case the spacecraft shall maneuver to rotate the component away from significant heat sources, typically the Sun. Given the temperature of a component, $T$, the temperature constraint is defined simply as,
% \begin{equation}
%     h_{temp}(\bm{x}) = T_{max}-T
% \end{equation}
% This constraint is relative degree 3 and could be enforced using HOCBFs; however, the Sun and Earth incidence angles with the surface are added to achieve better performance. The constraint is then given as,
% \begin{equation}
%     \Psi_{temp}({\bm{x}}) = T_{max}-T-\delta_0(\frac{\pi}{2}-\theta_{SI})-\delta_1(\frac{\pi}{2}-\theta_{EI})
% \end{equation}
% where $\delta_0$ and $\delta_1$ are constant coefficients that are tuned external to the QP and $T_{max}$ is the maximum allowable temperature. This constraint is relative degree 2, where HOCBFs are then used to transform $\Psi_{temp}$ into a valod CBF. Note that when $\theta_{SI} > 90\:deg$ and $\theta_{EI}>90 \:deg$, the gradient of the constraint is zero. However, in this case, temperature is decreasing and is not approaching $T_{max}$, so the CBF is valid. For this simulation, $T_{max}=10\: ^o C$ and $T$ is measured on the side of the spacecraft pointing along the $-y_B$ axis.
% \subsubsection{Maintain Battery Charge}
% The spacecraft shall maintain attitude requirements for sufficient power generation. For example, the spacecraft shall point its solar panels towards the sun to ensure the battery remains charged. Given the battery energy, $E$, the battery charge constraint is defined simply as,
% \begin{equation}
%     h_{batt}({\bm{x}}) = E-E_{min}
% \end{equation}
% where $E_{min}$ is the minimum allowable energy level, determined such that at this point the spacecraft would be able to maintain minimum function as determined by the mission. This constraint is relative degree 3. In this case, note that the gradient of the constraint is zero when the sun incidence angle with the side of spacecraft with the solar panels, $\theta_{SI}$, is greater than $90\:deg$. Therefore HOCBFs cannot be used to enforce this constraint. To account for this, $\theta_{SI}$ is added to the constraint, which is then given by,
% \begin{equation}
%     \Psi({\bm{x}}) = E-E_{min}-\delta_2\theta_{SI}
% \end{equation}
% This constraint is relative degree 2, where HCBFs are then used to transform it into a valid CBF. For this simulation, $E_{min}=1\:kJ$, and solar panels are assumed to cove the side of the spacecraft pointing along the $+z_B$ axis.
% \subsubsection{Avoid Actuation Saturation}
% The spacecraft actuation strategy shall conserve actuator use to prevent wear when possible. This constrain is not enforced with RTA, but rather is implemented as the admissible control set ${\mathcal{U}}$. For this simulation, $\dot{\psi}_{max}=181.3\:rad/s^2$ and ${\mathcal{U}}=[-\dot{\psi}_{max},\dot{\psi}_{max}]^3$.
% \subsubsection{Avoid Aggressive Maneuvering}
% The spacecraft shall maneuver below a threshold to prevent structural damage. For example, if the spacecraft rotates too quickly components might break. This constraint enforces limits on the angular velocity, $\bm{\omega}$, and angular acceleration, $\dot{\bm{\omega}}$, as well as the reaction wheel velocity, $\bm{\phi}$. The constraints for angular velocity and reaction wheel velocity are defined as,
% \begin{equation}
%     h_{\omega}({\bm{x}})=\omega_{max}^2-\omega^2
% \end{equation}
% \begin{equation}
%     h_{\psi}({\bm{x}})=\psi_{max}^2-\psi^2
% \end{equation}
% These constraints are relative degree 1 and are valid CBFs. Since the angular acceleration is not a state, it must be enforced differently. Given the system dynamics, $\dot{\omega}$ is directly related to $\dot{\phi}$ and $\omega$, so additional bounds for $\dot{\phi}_{max}$ can be used to enforce the constraint. The maximum angular acceleration occurs when ${\bm{\omega}} = [\omega_{max}]^3$ and  ${\dot{\bm{\omega}}} = [\dot{\omega}_{max}]^3$. From the system dynamics in Eq. \ref{e:full_dynamics}, enforcing the following constraints ensures that $|\dot{\omega}|\leq \dot{\omega}_{max}$,
% \begin{equation}
% \begin{split}
%     |\dot{\psi}_1| \leq \frac{J_1\dot{\omega}_{max} - |J_2-J_3|\omega_{max}^2}{D} \\
%     |\dot{\psi}_2| \leq \frac{J_2\dot{\omega}_{max} - |J_3-J_1|\omega_{max}^2}{D} \\
%     |\dot{\psi}_3| \leq \frac{J_3\dot{\omega}_{max} - |J_1-J_2|\omega_{max}^2}{D}
%     \end{split}
% \end{equation}
% These constraints are enforced as additional bounds on the admissible control set ${\mathcal{U}}$. For this simulation, $\dot{\omega}_{max} = 2\:deg/s^2$, $\omega_{max}=1\:deg/s$, and $\phi_{max}=576\:rad/s$.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Simulation Results}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This section presents the results of a simulation developed to test the constraints outlined in Section \ref{s:constraints}, where ASIF RTA is used to assure safety. This simulation uses the Safe Autonomy Run Time Assurance Framework \cite{ravaioli2023universal}, which simplifies user effort and supports automatic differentiation of all constraints, becoming particularly useful for the constraints that utilize HOCBFs.
% \subsection{Monte-Carlo Analysis}
% To verify that the RTA works regardless of initial conditions, a Monte-Carlo experiment was conducted. The simulations initialize random initial conditions that are with in the safe set, meaning no constraints are violated. To prevent a state being initialized on the constraint boundary, a $5\%$ buffer is added. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Conclusions}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \appendices{}              % note there is no {} to put a title. Each appendix has its own title
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % For a single appendix, use the \appendix{} keyword and do not use the \section command.

% \section{More Information}        % first appendix
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% This is the first appendix. 

% \subsection{Comments}
% If you have only one appendix, use the ``appendix'' keyword.

% \subsection{More Comments}
% Use section and subsection keywords as usual.

% \section{Yet More Information}    % second appendix
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This is the second appendix.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \acknowledgments


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \bibliographystyle{IEEEtran}
% %\bibliography{IEEEabr,MyBibFile}
% \bibliography{references}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \thebiography
% %% This biostyle allows you to insert your photo size 1in X 1.25in
% \begin{biographywithpic}{Kerianne L. Hobbs}{Figures/HobbsKerianne8x10}
% is the Safe Autonomy and Space Lead on the Autonomy Capability Team (ACT3) at the Air Force Research Laboratory. There she investigates rigorous specification, analysis, bounding, and intervention techniques to enable safe, trusted, ethical, and certifiable autonomous and learning controllers for aircraft and spacecraft applications. Her previous experience includes work in automatic collision avoidance and autonomy verification and validation research. Dr. Hobbs was selected for the 2020 AFCEA 40 Under 40 award and was a member of the team that won the 2018 Collier Trophy (Automatic Ground Collision Avoidance System Team), as well as numerous AFRL Awards.  Dr. Hobbs has a BS in Aerospace Engineering from Embry-Riddle Aeronautical University, an MS in Astronautical Engineering from the Air Force Institute of Technology, and a Ph.D. in Aerospace Engineering from the Georgia Institute of Technology. 
% \end{biographywithpic}




% \end{document}

==> reinforcement_learning.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Reinforcement Learning Control Law} \label{s:RL}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\todo{Reach out to Nate and he will gladly help write this section}
Brief intro to RL and how the control law is implemented via NN

\todo{edit the following copied from Nate:}
\emph{Reinforcement Learning} (RL) is a form of machine learning in which an agent acts in an environment, learns through experience, and increases its performance based on rewarded behavior. \emph{Deep Reinforcement Learning} (DRL) is a newer branch of RL in which a neural network is used to approximate the behavior function, i.e. policy $\policy$. The basic construction of the DRL approach is shown in \todo{figure for RL}. The agent consists of the \emph{Neural Network Controller} (NNC) and RL algorithm, and the environment consists of a plant and observer model. The environment can be comprised of any dynamical system, from Atari simulations (\cite{hamilton2020sonic, alshiekh2018safe}) to complex robotics scenarios (\cite{brockman2016openai, fisac2018general, henderson2018deep, mania2018simple, jang2019simulation, bernini2021few}). 

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.75\columnwidth]{images/rl_basic (2).png}
%     \caption{Basic formulation of Deep Reinforcement Learning for a control problem.}
%     \label{fig:drl_basic}
% \end{figure}

Reinforcement learning is based on the \textit{reward hypothesis} that all goals can be described by the maximization of expected return, i.e. the cumulative reward \cite{silver2015}. During training, the agent chooses an action, $\action_t$, based on the input observation, $\obs$. The action is then executed in the environment, which causes the environment to transition to state $\state_{t+1}$ with probability $\Transition(\state_t, \action_t, \state_{t+1})$ according to the plant model. However, instead of receiving the state information, the agent receives an observation $\obs_{t+1} \in \Obs$  which depends on the new state of the environment, $\state_{t+1}$, and on the just taken action, $\action_t$, with probability $\ObsFunc(\obs_{t+1} \mid \state_{t+1}, \action_t)$. Finally, the agent receives a reward $\reward_t$ equal to $\Reward(\state_t, \action_t, \state_{t+1})$.

The solution RL finds is the optimal behavior function, $\action = \policy^*(\state)$, that maximizes the expected cumulative sum of rewards, i.e. \textit{return}, $\Returnvar$:
\begin{equation}
    \label{eq:return}
    {\mathbb{E}} [\Returnvar] = {\mathbb{E}} [\sum_{t=0}^{\Horizon}\gamma^{t} \reward_t],
\end{equation}
where $\Horizon$ is a finite time-horizon. When $\gamma = 0$, the solution prioritizes immediate reward, and when $\gamma = 1$ the solution prioritizes maximizing the expected sum of future rewards.

\subsection{Proximal Policy Optimization}
Proximal Policy Optimization (PPO) was first introduced by Schulman et al. in \cite{schulman2017proximal} as an improvement to their previous DRL algorithm, \textit{Trust Region Policy Optimization} (TRPO) \cite{schulman2015trust}. Both algorithms are on-policy and focus on iteratively improving the policy in small increments to prevent against making large changes in the policy that might lead to a drop in performance. They differ in how the ``small increment'' is calculated. TRPO solves an optimization problem to identify the largest change to the policy that can be made while remaining within a ``trustworthy'' region. Solving this optimization problem is computationally expensive, so PPO simplifies the process using a clipping function. Instead of defining the trustworthy region based on the optimization problem, the clipping function sets a hard, constant limit. This simplification speeds up computation, and, according to the introductory paper, improves sample complexity. Later work, \cite{engstrom2019implementation}, showed that the improvements were actually a result of code-level improvements. Despite this finding, PPO has continued to grow and is regularly improved with new features.
\todo{end copied}
